Beyond NED: Fast and Effective Search Space Reduction for Complex Question Answering over Knowledge Bases

Answering complex questions over knowledge bases (KB-QA) faces huge input data with billions of facts, involving millions of entities and thousands of predicates. For efficiency, QA systems first reduce the answer search space by identifying a set of facts that is likely to contain all answers and relevant cues. The most common technique for doing this is to apply named entity disambiguation (NED) systems to the question, and retrieve KB facts for the disambiguated entities. This work presents CLOCQ, an efficient method that prunes irrelevant parts of the search space using KB-aware signals. CLOCQ uses a top-k query processor over score-ordered lists of KB items that combine signals about lexical matching, relevance to the question, coherence among candidate items, and connectivity in the KB graph. Experiments with two recent QA benchmarks for complex questions demonstrate the superiority of CLOCQ over state-of-the-art baselines with respect to answer presence, size of the search space, and runtimes.

==> sections/references.tex <==

General
- Stanford NLP tools
- Stanford NER (stanza)
- NLTK library
- LSH methods
- Wiki2vec paper
- Yago2 KG
- Lucene
- ElasticSearch

KG-encodings
- KOGNAC paper?
- HDT paper
- Adaptive Low-level Storage of Very Large Knowledge Graphs
- C.Weiss et al. Hexastore: Sextuple Indexing for Semantic Web Data Management. PVLDB, 1(1), 2008.
- Don’t Like RDF Reification? Making Statements about Statements Using Singleton Property WWW 2014

Top-k query processing
- Examining the Additivity of Top-k Query Processing Innovations. CIKM 2020: 1085-1094
-> https://dl.acm.org/doi/pdf/10.1145/3340531.3412000
-> recent, includes many references

- Pruned query evaluation using pre-computed impacts. SIGIR 2006: 372-379
-> Vo Ngoc Anh, Alistair Moffat:
-> key paper to cite, Moffat calls "score-ordered" lists "impact-ordered" - impact on the final ranking

- Vo Ngoc Anh, Alistair Moffat:
-> Pruning strategies for mixed-mode querying. CIKM 2006: 190-197
-> consider as well

- C. Buckley, A. F. Lewit: Optimization of Inverted Vector Searches, SIGIR 1985.
-> classical paper, confusing terminology, but close to Fagin-TA
-> Early threshold algorithm, avoids random accesses (FA does not avoid these)

- A survey of top-k query processing techniques in relational database systems. ACM Comput. Surv. 40(4): 11:1-11:58 (2008)
-> Ihab F. Ilyas, George Beskales, Mohamed A. Soliman:
-> best source on rank joins from a DB perspective, complementary to IR

- EASE: An Effective 3-in-1 Keyword Search Method for Unstructured, Semi-structured and Structured Data

- Top-X paper
- Efficient and self-tuning incremental query expansion for top-k query processing paper

Top-k query processing on KG
- Quark-X: An Efficient Top-K Processing Framework for RDF Quad Stores https://dl.acm.org/doi/pdf/10.1145/2983323.2983727
- CONVEX
- D.Wang et al. Top-k Queries on RDF Graphs. Information Sciences,316,2015.



USING HDT: vakulenko2019message


NED
- AIDA
- TagMe
- S-MART
not explicit ned, e.g. AQQU, MaSP; multi-task setups, QAmp: message passing, text-ray
one-shot, some allow top-k but commercial, some papers that do on own, KEQA->own module
 

Top-k


Benchmarks
- LC QuAD 2.0 paper
- CONVEX paper

QA
- PullNet
- Stagg
- Aqqu
- Quint
- Qamp - Vakulenko et al. 2019
- QAnswer
- Template-based Question Answering over RDF Data

Diefenbach et al 2019, QAnswer => using HDT

TAGME + KG (QA system that ELQ uses)


Look at AQQU CN

Facebook AI paper on unified KG+text qa mentions problems with qualifiers (entities in 2-hop!)
